Cats or CAT scans: transfer learning from natural or medical image source datasets?

Transfer learning is a widely used strategy in medical image analysis. Instead of only training a network with a limited amount of data from the target task of interest, we can first train the network with other, potentially larger source datasets, creating a more robust model. The source datasets do not have to be related to the target task. For a classification task in lung CT images, we could use both head CT images, or images of cats, as the source. While head CT images appear more similar to lung CT images, the number and diversity of cat images might lead to a better model overall. In this survey we review a number of papers that have performed similar comparisons. Although the answer to which strategy is best seems to be "it depends", we discuss a number of research directions we need to take as a community, to gain more understanding of this topic.

==> _draft.tex <==

\cite{kornblith2018better} study transfer of 13 networks in 12 image classification datasets. One of the important findings is that when the target data is fine-grained (as could be the case in medical imaging), networks trained from scratch perform similarly to networks pretrained on Imagenet.

\cite{recht2018cifar} use two independent parts of CIFAR-10 to demonstrate that the way performances are reported may not be representative of one method being superior over the other, and susceptible to even small changes in the distributions of the data.

\cite{azizpour2015generic} investigate transfer from Imagenet and Places to a range of computer vision tasks in 15 datasets. They find that transfer is more successful when the source and target datasets are similar, where similarity is defined more by the label space (for example, whether the categories are fine-grained) than the images themselves. In contrast to \todo{who was it}, they find that Places leads to worse results than Imagenet on fine-grained tasks. 

\cite{mahajan2018exploring} Transfer from (subsets of) 3 billion Instagram images to (subsets of) computer vision datasets. They find that the number of classes important, better results if better match between source and target task.

